LaMP-Cap: Personalized Figure Caption Generation With Multimodal Figure Profiles

Figure captions are crucial for helping readers understand and remember a figure's key message. Many models have been developed to generate these captions, helping authors compose better quality captions more easily. Yet, authors almost always need to revise generic AI-generated captions to match their writing style and the domain's style, highlighting the need for personalization. Despite language models' personalization (LaMP) advances, these technologies often focus on text-only settings and rarely address scenarios where both inputs and profiles are multimodal. This paper introduces LaMP-Cap, a dataset for personalized figure caption generation with multimodal figure profiles. For each target figure, LaMP-Cap provides not only the needed inputs, such as figure images, but also up to three other figures from the same document--each with its image, caption, and figure-mentioning paragraphs--as a profile to characterize the context. Experiments with four LLMs show that using profile information consistently helps generate captions closer to the original author-written ones. Ablation studies reveal that images in the profile are more helpful than figure-mentioning paragraphs, highlighting the advantage of using multimodal profiles over text-only ones.

==> table/table_main_study-byCategory.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{\textbf{Paper Category}} & \multicolumn{4}{c}{\textbf{BLEU}} & \multicolumn{3}{c}{\textbf{ROUGE}} \\ \cline{2-8} 
 & \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
\begin{tabular}[c]{@{}c@{}}Physics \\ (n=73,452)\end{tabular} & .300 & .212 & .164 & .132 & .414 & .215 & .333 \\ \hline
\begin{tabular}[c]{@{}c@{}}Comp Sci\\ (n=56,988)\end{tabular} & .312 & .236 & .192 & .160 & .413 & .238 & .365 \\ \hline
\begin{tabular}[c]{@{}c@{}}Maths\\ (n=6,120)\end{tabular} & .310 & .236 & .195 & .163 & .405 & .238 & .361 \\ \hline
\begin{tabular}[c]{@{}c@{}}EE and SS\\ (n = 4,092)\end{tabular} & .326 & .249 & .205 & .172 & .425 & .253 & .378 \\ \hline
\begin{tabular}[c]{@{}c@{}}Stats\\ (n=3,228)\end{tabular} & \multicolumn{1}{l}{.302} & \multicolumn{1}{l}{.224} & \multicolumn{1}{l}{.181} & \multicolumn{1}{l}{.151} & \multicolumn{1}{l}{.414} & \multicolumn{1}{l}{.231} & \multicolumn{1}{l}{.349} \\ \hline
\begin{tabular}[c]{@{}c@{}}Quant Bio \\ (n=1,500)\end{tabular} & \multicolumn{1}{l}{.289} & \multicolumn{1}{l}{.208} & \multicolumn{1}{l}{.166} & \multicolumn{1}{l}{.135} & \multicolumn{1}{l}{.403} & \multicolumn{1}{l}{.215} & \multicolumn{1}{l}{.329} \\ \hline
\begin{tabular}[c]{@{}c@{}}Quant Fina \\ (n=900)\end{tabular} & \multicolumn{1}{l}{.333} & \multicolumn{1}{l}{.255} & \multicolumn{1}{l}{.210} & \multicolumn{1}{l}{.176} & \multicolumn{1}{l}{.433} & \multicolumn{1}{l}{.256} & \multicolumn{1}{l}{.376} \\ \hline
Econ (n=169) & \multicolumn{1}{l}{.376} & \multicolumn{1}{l}{.293} & \multicolumn{1}{l}{.244} & \multicolumn{1}{l}{.203} & \multicolumn{1}{l}{.488} & \multicolumn{1}{l}{.302} & \multicolumn{1}{l}{.425} \\ \hline
\end{tabular}
\caption{Performance comparison of LLMs among different paper categories.}
\label{tab:main-result-byCategory}
\end{table}

==> table/table_main_study-byType.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{\textbf{Figure Type}} & \multicolumn{4}{c}{\textbf{BLEU}} & \multicolumn{3}{c}{\textbf{ROUGE}} \\ \cline{2-8} 
 & \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
Graph Plot \\ (n=93,900) & .316 & .231 & .184 & .151 & .425 & .235 & .356 \\ \hline
Node Diagram \\ (n=20,520) & .275 & .205 & .164 & .135 & .371 & .205 & .327 \\ \hline
Scatterplot \\ (n=12,024) & .296 & .208 & .161 & .129 & .409 & .210 & .328 \\ \hline
Bar Chart \\ (n=10,285) & .302 & .217 & .170 & .138 & .414 & .219 & .352 \\ \hline
Equation \\ (n=8,772) & \multicolumn{1}{l}{.280} & \multicolumn{1}{l}{.211} & \multicolumn{1}{l}{.170} & \multicolumn{1}{l}{.141} & \multicolumn{1}{l}{.381} & \multicolumn{1}{l}{.214} & \multicolumn{1}{l}{.335} \\ \hline
\end{tabular}
\caption{Performance comparison of LLMs among different figure type as target figure.}
\label{tab:main-result-byType}
\end{table}

==> table/table_main_study_2orMoreProfiles.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}
% \footnotesize
% \setlength{\tabcolsep}{2pt}
% \centering
% \begin{tabular}{@{}l@{\hspace{1pt}}l@{\hspace{1pt}}cccc@{\hspace{2pt}}ccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Profile\\ Used\end{tabular}}} & \multicolumn{4}{c}{\textbf{BLEU}} & \multicolumn{3}{c}{\textbf{ROUGE}} \\ \cline{3-9} 
%  &  & \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}GPT-\\ 4o\end{tabular}}} & \textbf{One} & .281 & .189 & .139 & .105 & .386 & .181 & .315 \\ \cline{2-9} 
%  & \textbf{All} & .309 & .215 & .163 & .126 & .413 & .209 & .342 \\ \hline
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Llama \\ 4 Scout\end{tabular}}} & \textbf{One} & .373 & .295 & .248 & .212 & .482 & .303 & .425 \\ \cline{2-9} 
%  & \textbf{All} & .419 & .343 & .294 & .258 & .524 & .349 & .468 \\ \hline
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Gemini\\ 2.5 Flash\end{tabular}}} & \textbf{One} & .372 & .293 & .245 & .211 & .483 & .303 & .426 \\ \cline{2-9} 
%  & \textbf{All} & .419 & .342 & .294 & .257 & .526 & .354 & .473 \\ \hline
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}GPT-\\ 4o mini\end{tabular}}} & \textbf{One} & .287 & .204 & .157 & .123 & .399 & .209 & .328 \\ \cline{2-9} 
%  & \textbf{All} & .318 & .236 & .188 & .153 & .430 & .245 & .360 \\ \hline
% \end{tabular}
% \caption{Performance comparison of LLMs with different profile settings. On data only with 2 or more profiles available (n=6284)}
% \label{tab:main-result-2more}
% \end{table}


\begin{table}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\definecolor{lightgreen}{rgb}{0.9, 1.0, 0.9}
\definecolor{darkgreen}{rgb}{0.7, 0.9, 0.7}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{Profile}} & \multicolumn{4}{c}{\textbf{BLEU}} & \multicolumn{3}{c}{\textbf{ROUGE}} \\ 
\cmidrule(lr){3-6} \cmidrule(lr){7-9}
 & \textbf{Used} & \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ 
\midrule
\multirow{2}{*}{GPT-4o} 
 & \cellcolor{lightgreen}One & \cellcolor{lightgreen}.281 & \cellcolor{lightgreen}.189 & \cellcolor{lightgreen}.139 & \cellcolor{lightgreen}.105 & \cellcolor{lightgreen}.386 & \cellcolor{lightgreen}.181 & \cellcolor{lightgreen}.315 \\ 
 & \cellcolor{darkgreen}All & \cellcolor{darkgreen}.309 & \cellcolor{darkgreen}.215 & \cellcolor{darkgreen}.163 & \cellcolor{darkgreen}.126 & \cellcolor{darkgreen}.413 & \cellcolor{darkgreen}.209 & \cellcolor{darkgreen}.342 \\ 
\midrule
\multirow{2}{*}{Llama-4 Scout}
 &  \cellcolor{lightgreen}One & \cellcolor{lightgreen}.373 & \cellcolor{lightgreen}.295 & \cellcolor{lightgreen}.248 & \cellcolor{lightgreen}.212 & \cellcolor{lightgreen}.482 & \cellcolor{lightgreen}.303 & \cellcolor{lightgreen}.425 \\ 
 & \cellcolor{darkgreen}All & \cellcolor{darkgreen}.419 & \cellcolor{darkgreen}.343 & \cellcolor{darkgreen}.294 & \cellcolor{darkgreen}.258 & \cellcolor{darkgreen}.524 & \cellcolor{darkgreen}.349 & \cellcolor{darkgreen}.468 \\ 
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Gemini-2.5\\Flash Preview\end{tabular}} 
 & \cellcolor{lightgreen}One & \cellcolor{lightgreen}.372 & \cellcolor{lightgreen}.293 & \cellcolor{lightgreen}.245 & \cellcolor{lightgreen}.211 & \cellcolor{lightgreen}.483 & \cellcolor{lightgreen}.303 & \cellcolor{lightgreen}.426 \\ 
 & \cellcolor{darkgreen}All & \cellcolor{darkgreen}.419 & \cellcolor{darkgreen}.342 & \cellcolor{darkgreen}.294 & \cellcolor{darkgreen}.257 & \cellcolor{darkgreen}.526 & \cellcolor{darkgreen}.354 & \cellcolor{darkgreen}.473 \\ 
\midrule
\multirow{2}{*}{GPT-4.1 Mini}  
 & \cellcolor{lightgreen}One & \cellcolor{lightgreen}.287 & \cellcolor{lightgreen}.204 & \cellcolor{lightgreen}.157 & \cellcolor{lightgreen}.123 & \cellcolor{lightgreen}.399 & \cellcolor{lightgreen}.209 & \cellcolor{lightgreen}.328 \\ 
 & \cellcolor{darkgreen}All & \cellcolor{darkgreen}.318 & \cellcolor{darkgreen}.236 & \cellcolor{darkgreen}.188 & \cellcolor{darkgreen}.153 & \cellcolor{darkgreen}.430 & \cellcolor{darkgreen}.245 & \cellcolor{darkgreen}.360 \\ 
\bottomrule
\end{tabular}
\caption{Performance comparison of LLMs with different profile settings. On data only with 2 or more profiles available (n=6284)}
\label{tab:main-result-2more}
\end{table}

==> table/table_profile_config.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lll}
\toprule
\textbf{Config.} & \textbf{Target} & \textbf{Profile} \\ \hline
\multicolumn{1}{l|}{No-Profile} & \multicolumn{1}{l|}{Img + Para} & None \\ \hline
\multicolumn{1}{l|}{One-Profile} & \multicolumn{1}{l|}{Img + Para} & 1 profile (Img + Para + Cap) \\ \hline
\multicolumn{1}{l|}{All-Profile} & \multicolumn{1}{l|}{Img + Para} & All profiles (Img + Para + Cap) \\ 
\bottomrule
\end{tabular}
\caption{Input settings for each configuration in the generation task.}
\label{tab:config}
\end{table}
